Computation in Coxeter groups II. Minimal roots

In the recent paper (Casselman, 2001) I described how a number of ideas due to Fokko du Cloux and myself could be incorporated into a reasonably efficient program to carry out multiplication in arbitrary Coxeter groups. At the end of that paper I discussed how this algorithm could be used to build the reflection table of minimal roots, which could in turn form the basis of a much more efficient multiplication algorithm. In this paper, following a suggestion of Bob Howlett, I explain how results due to Brigitte Brink can be used to construct the minimal root reflection table directly and more efficiently.

==> inputs/refs.tex <==

\newcount\refno
\refno=0
\def\refitem{\medskip
\advance\refno by 1
{\bold \the\refno. }}
\def\jour#1{{\frenchspacing \sl #1}}
\def\pp#1{{\frenchspacing #1}}
\def\article#1{`#1'}
\def\book#1{{\sl #1}}
\def\vol#1{{\bold #1}}


==> satzlbls.tex <==
\expandafter \def \csname satzProposition\endcsname {Proposition 1.1}
\expandafter \def \csname satzCorollary\endcsname {Corollary 1.2}
\expandafter \def \csname satzLemma\endcsname {Lemma 1.3}
\expandafter \def \csname satzProposition\endcsname {Proposition 1.4}
\expandafter \def \csname satzLemma\endcsname {Lemma 1.5}
\expandafter \def \csname satzProposition\endcsname {Proposition 1.6}
\expandafter \def \csname satzLemma\endcsname {Lemma 1.7}
\expandafter \def \csname satzCorollary\endcsname {Corollary 1.8}
\expandafter \def \csname satzCorollary\endcsname {Corollary 1.9}
\expandafter \def \csname satzLemma\endcsname {Lemma 2.1}
\expandafter \def \csname satzLemma\endcsname {Lemma 3.1}
\expandafter \def \csname satzProposition\endcsname {Proposition 3.2}
\expandafter \def \csname satzProposition\endcsname {Proposition 4.1}
\expandafter \def \csname satzCorollary\endcsname {Corollary 4.2}
\expandafter \def \csname satzCorollary\endcsname {Corollary 4.3}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.1}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.2}
\expandafter \def \csname satzCorollary\endcsname {Corollary 5.3}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.4}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.5}
\expandafter \def \csname satzLemma\endcsname {Lemma 5.6}
\expandafter \def \csname satzLemma\endcsname {Lemma 5.7}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.8}
\expandafter \def \csname satzProposition\endcsname {Proposition 5.9}
\expandafter \def \csname satzProposition\endcsname {Proposition 6.1}
\expandafter \def \csname satzLemma\endcsname {Lemma 6.2}
\expandafter \def \csname satzProposition\endcsname {Proposition 6.3}
\expandafter \def \csname satzProposition\endcsname {Proposition 6.4}
\expandafter \def \csname satzProposition\endcsname {Proposition 6.5}

